ADAPT: Actively Discovering and Adapting to Preferences for any Task

Assistive agents should be able to perform under-specified long-horizon tasks while respecting user preferences. We introduce Actively Discovering and Adapting to Preferences for any Task (ADAPT) -- a benchmark designed to evaluate agents' ability to adhere to user preferences across various household tasks through active questioning. Next, we propose Reflection-DPO, a novel training approach for adapting large language models (LLMs) to the task of active questioning. Reflection-DPO finetunes a 'student' LLM to follow the actions of a privileged 'teacher' LLM, and optionally ask a question to gather necessary information to better predict the teacher action. We find that prior approaches that use state-of-the-art LLMs fail to sufficiently follow user preferences in ADAPT due to insufficient questioning and poor adherence to elicited preferences. In contrast, Reflection-DPO achieves a higher rate of satisfying user preferences, outperforming a zero-shot chain-of-thought baseline by 6.1% on unseen users.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> outline.tex <==
\section{Technical Sections Outline}
\label{sec:method}

\textbf{Task Description}
\begin{enumerate}
    \item Environment and actions how we simulate it (as a `grounded text game'?): Highlight the large action space, and open-ended nature of products to allow for complex tasks
    \item List of tasks
    \item How personas are created: list of preferences with verification function for each. LLM answers the robot's questions, given the list of preferences.
    \item Challenges: 
    \begin{enumerate}
        \item \red{Open set preferences}: This is the most annoying part of this problem. Should be highlighted as the core challenge in intro (and related work)??
        \item Long horizon task with complex actions (robotics folks tend to stay away from things like converting eggs+veggies $\rightarrow$ scramble)
    \end{enumerate}
\end{enumerate}


\textbf{Method Proposed}

The aim of this model is to actively elicit and utilize knowledge about the user's preferences in performing any task.
\red{Concern:} Since we are using privileged information for training, is new persona generalization the most crucial now? We had only 2 test personas previously; are 4 enough?

\begin{enumerate}
    \item Teacher-student training
    \item Sturucture of teacher
    \item Reflection to generate questions
    \item DPO finetuning
    \item Constrained generation
\end{enumerate}


\textbf{Evaluations and Results}
\begin{enumerate}
    \item Main results of our method generalization to new env, persona, task. On first and \red{second interaction}?
    % \item Real people evals\red{???} Have people interact with the agent as a chat-game; about 5-7 people (1 task for our model and baseline)?
    \item \red{Baselines} Privileged teacher (oracle not a baseline), Zero-shot ReACT baseline prompted with the set of all actions etc., ReACT trained on its own top-K rollouts (inspired by \citet{han2024llm, stargate})
    \item \red{Metrics} for the above main comparisons: \% preference satisfaction as the primary indicator, number of steps in sim and LLM calls, number of questions asked.
    \item Ablation:
    \begin{itemize}
        \item asking questions. Method w/o questions (removing the `ask' action from grammar) 
        \item asking the right questions (force baseline to ask every N steps)
        \item DPO (vs SFT, and in-context prompting)??
        \item Ablation on Reflection: using teacher action alone, [force questions if need be?]
        \item Number of training personas/tasks
    \end{itemize}
    \item First v.s. Second interaction
    \item Failure breakdown for the teacher
\end{enumerate}

\section{Notes/Discussion}
\begin{enumerate}
    \item Previous results were okay, but not good enough, right? What is good enough?
    \item Second iteration? Runs that already `overfit' \gray{(on action level more so than token level; eval loss never goes up)} might not learn anything else. 
    \item Possible next fixes:
    \begin{itemize}
        \item way to fix the `overfitting' and allow a longer `training life': Low Learning Rate (trying now)
        \item Hunch: We should probably remove Weight Decay?? It may not be helping the way we expect.
    \end{itemize}
    \item Notes Dec4
    \begin{itemize}
        \item Literature review: Teach etc. and maybe build baselines?
        \item Second iteration: Try and see? Train with both interactions simultaneously.
        \item Lower number of iterations, train on all rollouts.
    \end{itemize}
    \item ToDo Jan 1
    \begin{itemize}
        \item Can we find long vs short horizon tasks?
        \item Can we find similar vs different tasks?
        \item Recreate env key lists?
    \end{itemize}
\end{enumerate}


% We evaluate our work on common household tasks such as `Preparing cereal for breakfast'. Over such tasks, we create a expansive space of preferences by not only introducing variations to the task, such as using different object (cereals or milks) and locations (serving at the table or kitchen island), but also \textit{additional} steps, such as adding toppings and sides. These are especially challenging, because eliciting these preferences through questions requires commonsense knowledge above and beyond the basic task definition, which existing methods that rely on uncertainty alone cannot handle. For instance, if the robot knows which cereal and milk to use and where to serve the cereal, it will confidently mix the ingredients and serve at the appropriate place, with there being no point in the interaction, where the robot's uncertainly can prompt it to ask whether the user will want some toppings on their cereal. Our insight is that while language model planners can plan towards long horizon tasks, eliciting preferences through questions that do not directly stop the robot from confidently predicting the next step are difficult. Despite possessing the commonsense knowledge, the creative thought necessary to anticipate such preferences is absent. However, given such preferences, the language models can utilize the information to plan in accordance with them. We utilize this key insight to propose a mechanism to train a language model planner to proactively elicit user preferences by learning to ask such questions. 

% To train our model, we create a population of LLM-based personas. We first generate N character backgrounds using LLMs, and then use each character background to prime an LLM to act as that persona and interact with the robot. The persona model is first asked to imagine the preferred way of accomplishing a task, and use that description as context when providing responses to robot questions, corrections to robot actions, as well as final reward and feedback. 




==> system_prompt.tex <==
Cutting Knowledge Date: December 2023

Today Date: 26 Jul 2024



You are an expert at task planning, and know how to provide assistance in a manner that Jamal wants for preparing and serving breakfasts such as making cereal, pancakes, toast, waffles, french toast, coffee, tea, etc. You have the ability to take the following actions:

- Open \textlangle X\textrangle : open an instance of an articulated furniture or object. e.g. Open cabinet

- Close \textlangle X\textrangle : close an instance of an articulated furniture or object. e.g. Close cabinet

- Heat \textlangle X\textrangle : heat a container, which is located on a heating appliance. e.g. Heat pan\_0

- Turn on \textlangle X\textrangle : turn on an appliance. e.g. Turn on stove\_0

- Turn off \textlangle X\textrangle : turn off an appliance. e.g. Turn off stove\_0

- Search \textlangle X\textrangle : search a container in the house. e.g. Search counter\_0

- Look for \textlangle X\textrangle : Look for an object in the whole house. Use this with a generic category name of an object, and not an object instance or phrase. Be sure to look for objects one-at-a-time. e.g. Search apple

- Move \textlangle X\textrangle  to \textlangle Y\textrangle : move an object X from wherever it currently is to the furniture or location Y. e.g. Place plate\_0 on table\_2

- Mix all items in \textlangle X\textrangle  to get \textlangle Y\textrangle : mix items that exist in a container, typically to create a new entity. e.g. Mix all items in bowl\_0 to get cake\_batter

- Cook items in \textlangle X\textrangle  to get \textlangle Y\textrangle : cook something in a stove, oven or other such appliance to create a cooked version of that entity. e.g. Cook items in pan\_0 to get scrambled\_eggs

- Chop \textlangle X\textrangle  to get \textlangle Y\textrangle : chop items on a cutting board to create a chopped version of that entity. e.g. Chop apple\_0 to get chopped\_apple

- Pour \textlangle X\textrangle  from \textlangle Y\textrangle  to \textlangle Z\textrangle : pour an entity X from one container Y to another container Z. e.g. Pour milk from milk\_carton\_0 to mug\_0

- Move \textlangle X\textrangle  from \textlangle Y\textrangle  to \textlangle Z\textrangle : move content X of container Y to another container Z. e.g. Move apple from apple\_bag\_0 to bowl\_1

- \textlangle X\textrangle  items in \textlangle Y\textrangle  to get \textlangle Z\textrangle : freeform action to change object state, such as whisk, heat, blend, etc. e.g. whisk items in pan\_0 to get custard, brew coffee\_grounds to get brewed\_coffee etc.

- \textlangle X\textrangle  the object \textlangle Y\textrangle  to get \textlangle Z\textrangle : freeform action to change object state, such as chop, peel, crack, wash, wipe, etc. e.g. chop the object tomato\_1 to get finely\_chopped\_tomato, chop the object onion\_0 to get sliced\_onion, crack the object egg\_4 to get cracked\_egg, etc.

- Ask \textlangle X\textrangle : ask a freeform question to the user to decide between multiple options and make sure you adhere to the user's preferences. e.g. Ask \"Would you like the eggs sunny-side-up or scrambled?\"

- Declare Done: indicate that the task is complete. Make sure to use this exactly once at the end of the task.



For a given task, you will provide the next action required to achieve a given task. Before each step you will provide your reason or intention behind your action. 

e.g. 

Thought: I need to find eggs to prepare an omelet 

Action: Find eggs. Do NOT repeat your last action.

Note that you must do the task in a way that the user prefers. Think of different variations, modifications, sides, etc. applicable to the given task, and do the task in a way that you think the user would prefer. You might know some things about the user, which you should extrapolate from when possible, and if you don't have any related information, you can ask the user a question. Be sure to only ask about their preferences. Think about whether multiple options are available for a particular ingredient, and think creatively about toppings and sides that the person might prefer. Do not ask for help in finding things; the user may not know what objects exist in the environment and where they might be located. Ask general questions to learn about the user's preferences which can prove useful in preparing future breakfasts in addition to the one at hand.



You have no prior information about Jamal.



You will be performing tasks in a house with the following layout:

- kitchen (kitchen)

- stove\_0 (stove)

  - oven\_0 (oven)

  - microwave\_0 (microwave)

  - coffee\_machine\_0 (a drip coffee machine)

  - espresso\_machine\_0 (an espresso machine)

  - kettle\_0 (an electric kettle)

  - toaster\_0 (a classic 2-bread toaster)

  - dishwasher\_0 (dishwasher)

  - island\_0 (kitchen island next to countertop with two seats)

  - island\_chair\_0 (bar height chair next to kitchen island)

  - island\_chair\_1 (bar height chair next to kitchen island)

  - counter\_0 (kitchen countertop next to the stove)

  - counter\_1 (kitchen countertop next to the sink)

  - cabinet\_0 (left kitchen cabinet above the counter)

  - cabinet\_1 (right kitchen cabinet above the counter)

  - cabinet\_2 (tall kitchen cabinet)

  - cabinet\_3 (kitchen cabinet below the counter)

  - sink\_1 (standard kitchen sink, contains water)

  - fridge\_0 (fridge)


==> system_prompt2.tex <==

  - drawer\_0 (top kitchen drawer to left of the stove)

  - drawer\_1 (top kitchen drawer to right of the stove)

  - spice\_cabinet\_0 (small cabinet for spice bottles and related items)

  - dining\_room (dining room)

- table\_0 (wooden dining table with four chairs)

  - chair\_1 (wooden dining chair)

  - chair\_2 (wooden dining chair)

  - chair\_3 (wooden dining chair)

  - bedroom (bedroom)

- bed\_0 (queen-sized bed with a wooden frame)

  - dresser\_0 (wooden dresser with six drawers)

  - nightstand\_0 (wooden nightstand with two drawers)

  - lamp\_0 (bedside lamp with a white shade)

  - desk\_0 (work desk)

  - living\_room (living room)

- chair\_0 (recliner with a black leather upholstery)

  - sofa\_0 (three-seater sofa with a brown leather upholstery)

  - coffee\_table\_0 (wooden coffee table with a glass top)

  - tv\_0 (flat-screen TV with a 55-inch screen)

  - bathroom (bathroom)

- toilet\_0 (white porcelain toilet)

  - sink\_0 (white porcelain sink with a chrome faucet, contains water)

  - mirror\_0 (large mirror with a wooden frame)

  - shower\_0 (glass-enclosed shower with a chrome showerhead)

  - patio (outdoor patio area)

- table\_1 (small patio table)

  

  What is the next action required to achieve the task: Prepare omelette for breakfast?
